On the Dirichlet Problem for First Order Linear Hyperbolic PDEs on Bounded Domains with Mere Inflow Boundary

Here we study the Dirichlet problem for first order linear and quasi-linear hyperbolic PDEs on a simply connected bounded domain of $\R^2$, where the domain has an interior outflow set and a mere inflow boundary. By means of a Lyapunov function we show the existence of a unique solution in the space of functions of bounded variation and its continuous dependence on all the data of the linear problem. Finally, we conclude the existence of a solution to the quasi-linear case by utilizing the Schauder fixed point theorem. This type of problems considered here appears in applications such as transport based image inpainting.

==> macros.tex <==
%%
% at "@" und "!" als letter
%% 
\expandafter\edef\csname @catcode\endcsname{\the\catcode`\@}
\expandafter\edef\csname !catcode\endcsname{\the\catcode`\!}
\catcode`\@11
\catcode`\!11

%%%% skips
\smallskipamount=3pt plus 0.5pt minus 0.5pt
\medskipamount=6pt plus 1pt minus 1pt
\bigskipamount=12pt plus 2pt minus 2pt

%%% Tabellen
\renewcommand{\arraystretch}{1.5}

%%% Mengen
\def\A{{\mathcal{A}}}                 %% generische sigma-Algebra
\def\B{{\mathcal{B}}}                 %% Borel-sigma-Algebra
\def\Sk{{\mathcal{S}}} 		%% Skelett
\def\N{{\mathbb{N}}}                  %% natürliche Zahlen
\def\Z{{\mathbb{Z}}}                  %% ganze Zahlen
\def\R{{\mathbb{R}}}                  %% reellen Zahlen
\def\1{{\mathbb{1}}}			%% charakteristische Funktion
\def\Rinfty{\overline{\mathbb{R}} }         %% reellen Zahlen mit +infty und -infty


% meine Funktionenmengen
\def\FD{{\mathcal{F}}}                %% Functional domain general
\def\FR{{\mathcal{G}}}                %% Functional range general
\def\FF{{\mathfrak{F}}}                 %% Functional domain in L^1
\def\FX{{\mathfrak{X}}}                %%  Functional domain in BV
\def\FB{{\mathfrak{B}}}                %%  Randfunktionen aus BV  
                

%%% Parameter
\def\const{{\mathrm{const}}}          %% irgendeine Konstance

%%% Funktionenräume 
\def\C{C}                                      %% stetige Funktionen
\def\L{L}                                         %% Lebesgue intbare Funktionen
\def\Lloc{L_{\mathrm{loc}}}           %% lokal Lebesgue intbare Funktionen
\def\W{W}                                          %% Sobolev Raum
\def\BV{{\mathit{BV}}}                %% Funktionen beschr. Variation
\def\SBV{{\mathit{SBV}}}              %% spez. Funktionen beschr. Variation
\def\PT{{\mathit{P}}}                %% periodische Testfunktionen

%%% Maße
\def\Hm{{\mathcal{H}}}                %% Hausdorff-Maß
\def\Lm{{\mathcal{L}}}                %% Lebesgue-Maß
\def\Mloc{{\mathcal{M}_{\mathrm{loc}}}}%% vektorwertige Radon-Maße
\def\M{{\mathcal{M}}}                 %% endliche Radon-Maße

%% Verweis auf Gleichung
\def\refEq#1{(\ref{#1})}

%% Intervall
\def\IV#1#2,#3#4{\left#1#2,#3\right#4}
\def\usIV#1#2;#3#4{\mathopen{#1}#2;#3\mathclose{#4}}

%% Skalarprodukt / Norm
\def\SP#1#2,#3#4{\left#1#2,#3\right#4}
\def\Norm#1#2{\Vert#1\Vert_{#2}}                                   %% Norm
\def\sNorm#1#2{\left\Vert#1\right\Vert_{#2}}                 %% sNorm: norm mit left und right Skalierung
\def\genNorm#1{\Vert#1\Vert}                                          %% generische Norm

%% Operatoren
\def\arclength{\mathop{\operator@font arclength}}                       %% Bogenlänge
\let\bd\partial                                                                                          %% Rand, boundary
\let\pd\partial                                                                                          %% partial derivative
\let\cl\overline                                                                                         %% Abschluss closure
\def\div{\mathop{\operator@font div}}                                             %% Divergenz
\DeclareMathOperator{\dist}{dist}                              %% distance
\def\liminf{\mathop{\smash{\operator@font lim\,inf}}}        % liminf
\def\limsup{\mathop{\smash{\operator@font lim\,sup}}}        % limsup
\def\supp{\mathop{\smash{\operator@font supp}}}          % support
\def\O{\mathcal{O}}                                          % Landau
\def\o{{o}}                                                          % Landau klein
\def\Var{\mathop{\operator@font Var}}                        % Variation
\def\trace{\mathop{\operator@font trace}}                        % spur
\DeclareMathOperator{\sgn}{sgn}                                % signum
\DeclareMathOperator{\lingen}{span}                                % span
\def\inner#1{\mathring{#1}} 
\def\diam{\mathop{\operator@font diam}}                         %% Diameter

%%% binäre Operatoren
\def\longrightharpoonup{%                                    % long-Variante von rightharpoonup
  \relbar\joinrel\rightharpoonup
}
\let\wo\backslash                                            %% ohne
\let\nb\sim                                                  %% Nachbarschaft
\def\rto{\,\hbox{\vrule height7pt width0.5pt depth0pt        %% Restriktion
  \vrule height0.5pt width5pt depth0pt}\,}
\def\cc{\mathbin{\mathord{\subset}\!\mathord{\subset}}}        %% compact subset
\let\asymp\sim                                               %% asymptot. Verh.
\def\symdiff{\mathbin{\Delta}}                               %% symmetr. Diff.
\let\gdw\Leftrightarrow                                      %% genau dann wenn
\def\strongto{%                                              %% starke Konvergenz
  \@ifnextchar[\@strongto{\@strongto[]}}
\def\@strongto[#1]{%
  \def\temp{#1}%
  \ifx\temp\empty
  \to
  \else
  \mathrel{\mathop{\longrightarrow}\limits_{\scriptstyle#1}}%
  \fi
}
\def\weakto{%                                                % schwache Konvergenz
  \@ifnextchar[\@weakto{\@weakto[]}}
\def\@weakto[#1]{%
  \def\temp{#1}%
  \ifx\temp\empty
  \rightharpoonup
  \else
  \mathrel{\mathop{\longrightharpoonup}\limits_{\scriptstyle#1}}%
  \fi
}
\def\weaksto{%                                                % schwache* Konvergenz
  \@ifnextchar[\@weaksto{\@weaksto[]}}
\def\@weaksto[#1]{%
  \def\temp{#1}%
  \ifx\temp\empty
  \mathrel{\mathop{\rightharpoonup}\limits^{\scriptstyle*}}%
  \else
  \mathrel{\mathop{\longrightharpoonup}\limits^{\scriptstyle*}_{\scriptstyle#1}}%
  \fi
}
\let\symdiff\Delta                                            % symmetrische Differenz
\def\dotarg{\mathord{\, .\,}}                              % beliebiges Argument mit Punkt


%%
% Theoreme und Environments
%%


\newtheorem{theo}{Theorem}[section]
\newtheorem{lem}[theo]{Lemma}%[chapter]
\newtheorem{cor}[theo]{Corollary}%[chapter]
\newtheorem{prop}[theo]{Proposition}%[chapter]
\newtheorem{defi}[theo]{Definition}%[chapter]
\newtheorem{req}[theo]{Requirement}%[chapter]
\newtheorem{prob}[theo]{Problem}%[chapter]
\newtheorem{rem}[theo]{Remark}%[chapter]

%% Beweis:
%% Umbruch danach nicht unerwünscht
%\let\orig@end@proof\endproof
%\def\endproof{\orig@end@proof\penalty-500\relax}

%% Davor hat auch niemand was dagegen
%\let\orig@proof\proof
%\def\proof{\penalty-500 \orig@proof}


%% kein Absatz Einzug
%\parindent=0pt

%% dafür aber etwas Parskip zur Abtrennung verschiedener Absätze
%\parskip=3pt plus1.5pt minus1pt

%% die Ränder
\evensidemargin=2cm %54pt
\oddsidemargin=2cm %54pt

%\advance\evensidemargin -2.5mm
%\advance\oddsidemargin -2.5mm

%% marks für Headline
%\def\chaptermark#1{%
%  \markboth {%
%    \ifnum \c@secnumdepth >\m@ne
%      \if@mainmatter
%        \@chapapp\ \thechapter\enskip%
%      \fi
%    \fi
%    #1}{}}%
%\def\sectionmark#1{%
%  \markright {%
%    \ifnum \c@secnumdepth >\z@
%      \thesection\enskip%
%    \fi
%    #1}}

\endinput

